Berkeley Supernova Ia Program V: Late-Time Spectra of Type Ia Supernovae

In this work we analyse late-time (t > 100 d) optical spectra of low-redshift (z < 0.1) Type Ia supernovae (SNe Ia) which come mostly from the Berkeley Supernova Ia Program dataset. We also present spectra of SN 2011by for the first time. The BSNIP sample studied consists of 34 SNe Ia with 60 nebular spectra, to which we add nebular spectral feature measurements of 20 SNe Ia from previously published work (Maeda et al. 2011; Blondin et al. 2012), representing the largest set of late-time SN Ia spectra ever analysed. The full width at half-maximum intensity (FWHM) and velocities of the [Fe III] {\lambda}4701, [Fe II] {\lambda}7155, and [Ni II] {\lambda}7378 emission features are measured in most observations of spectroscopically normal objects where the data have signal-to-noise ratios >20 px^-1 and are older than 160 d past maximum brightness. The velocities of all three features are seen to be relatively constant with time, increasing only a few to ~20 km/s/d. The nebular velocity (v_neb, calculated by taking the average of the [Fe II] {\lambda}7155 and [Ni II] {\lambda}7378 velocities) is correlated with the near-maximum-brightness velocity gradient and early-time ejecta velocity. Nearly all high velocity gradient objects have redshifted nebular lines while most low velocity gradient objects have blueshifted nebular lines. No correlation is found between v_neb and {\Delta}m_15(B), and for a given light-curve shape there is a large range of observed nebular velocities. The data also indicate a correlation between observed (B-V)_max and v_neb.

==> final_vel.tex <==
\setlength{\tabcolsep}{0.05in}
\begin{table*}
\scriptsize
\begin{center}
\caption{Summary of objects studied. Uncertainties are given in parentheses.}\label{t:final_vel}
\begin{tabular}{lccccrrrcc}
\hline\hline
SN Name & $\Delta m_{15}(B)$$^\textrm{a}$ & Wang & Photospheric Vel.$^\textrm{c}$ & Benetti$^{\phantom{\textrm{dj}}}$ & \multicolumn{1}{c}{$\dot{v}$$^\textrm{e}$} & \multicolumn{1}{c}{$v_0$$^\textrm{f}$} & \multicolumn{1}{c}{Nebular Vel.$^\textrm{g}$} & EW(Na) & EW(Ca) \\
     & (mag) & Type$^\textrm{b}$ & ($10^3$~\kms) & Type$^{\textrm{d}\phantom{\textrm{j}}}$ & \multicolumn{1}{c}{(\kms~day$^{-1}$)} & \multicolumn{1}{c}{($10^3$~\kms)} & \multicolumn{1}{c}{(\kms)} & (\AA) & (\AA) \\
\hline

SN 1989M            &  1.10 (0.20) &     HV$\phantom{^\textrm{i}}$ &             12.46 (0.10)$\phantom{^\textrm{h}}$ &            HVG$\phantom{^\textrm{hj}}$ &                         291.84 (139.49)$\phantom{^\textrm{hj}}$ &                13.19 (0.42)$\phantom{^\textrm{hj}}$ &     $560$ $\phantom{0}$(110) & 1.88 (0.73) & 0.36 (0.18) \\
SN 1993Z            &     $\cdots$ & $\cdots\phantom{^\textrm{i}}$ &                 $\cdots$$\phantom{^\textrm{h}}$ &       $\cdots$$\phantom{^\textrm{hj}}$ &              \multicolumn{1}{c}{$\cdots\phantom{^\textrm{hj}}$} &  \multicolumn{1}{c}{$\cdots\phantom{^\textrm{hj}}$} &    $1990$ $\phantom{0}$(630) & 1.56 (0.40) & 0.96 (1.67) \\
SN 1994D$^\dagger$  &  1.36 (0.05) &      N$\phantom{^\textrm{i}}$ &             10.72 (0.10)$\phantom{^\textrm{h}}$ &            LVG$\phantom{^\textrm{hj}}$ &              33.43 $\phantom{00}$(6.77)$\phantom{^\textrm{hj}}$ &                10.60 (0.05)$\phantom{^\textrm{hj}}$ &   $-1720$ $\phantom{0}$(570) & 0.40 (0.44) & 0.09 (0.08) \\
SN 1998bu           &  1.05 (0.03) &      N$\phantom{^\textrm{i}}$ &                       10.84 (0.11)$^\textrm{h}$ & LVG$^{\textrm{h}\phantom{\textrm{j}}}$ &   46.52 $\phantom{00}$(5.38)$^{\textrm{h}\phantom{\textrm{j}}}$ &     11.01 (0.05)$^{\textrm{h}\phantom{\textrm{j}}}$ &   $-1800$ $\phantom{0}$(280) & 1.52 (1.12) & 0.39 (0.19) \\
SN 1999aa$^\dagger$ &  0.79 (0.05) &           $\cdots^\textrm{i}$ &             10.50 (0.10)$\phantom{^\textrm{h}}$ & LVG$^{\textrm{j}\phantom{\textrm{h}}}$ &   14.33 $\phantom{00}$(3.52)$^{\textrm{j}\phantom{\textrm{h}}}$ &     10.49 (0.03)$^{\textrm{j}\phantom{\textrm{h}}}$ &     $760$ $\phantom{00}$(70) & 0.44 (0.64) & 0.27 (0.14) \\
SN 1999gh$^\dagger$ &  1.69 (0.05) &      N$\phantom{^\textrm{i}}$ &             11.02 (0.10)$\phantom{^\textrm{h}}$ &          FAINT$\phantom{^\textrm{hj}}$ &              46.49 $\phantom{0}$(10.13)$\phantom{^\textrm{hj}}$ &                11.20 (0.13)$\phantom{^\textrm{hj}}$ &    $1570$ $\phantom{0}$(280) & 0.50 (0.25) &    $\cdots$ \\
SN 2002bo           &  1.15 (0.04) &     HV$\phantom{^\textrm{i}}$ &             13.88 (0.10)$\phantom{^\textrm{h}}$ &            HVG$\phantom{^\textrm{hj}}$ &             245.14 $\phantom{00}$(8.12)$\phantom{^\textrm{hj}}$ &                13.61 (0.09)$\phantom{^\textrm{hj}}$ &                 $2430$ (100) & 2.36 (0.53) & 0.57 (0.31) \\
SN 2002fk$^\dagger$ &  1.20 (0.03) &      N$\phantom{^\textrm{i}}$ & $\phantom{0}$9.51 (0.10)$\phantom{^\textrm{h}}$ & LVG$^{\textrm{j}\phantom{\textrm{h}}}$ &   11.21 $\phantom{00}$(8.28)$^{\textrm{j}\phantom{\textrm{h}}}$ &      9.74 (0.05)$^{\textrm{j}\phantom{\textrm{h}}}$ &   $-2060$ $\phantom{0}$(690) & 0.46 (0.09) & 0.26 (0.07) \\
SN 2003gs           &     $\cdots$ & $\cdots\phantom{^\textrm{i}}$ &                 $\cdots$$\phantom{^\textrm{h}}$ &       $\cdots$$\phantom{^\textrm{hj}}$ &              \multicolumn{1}{c}{$\cdots\phantom{^\textrm{hj}}$} &  \multicolumn{1}{c}{$\cdots\phantom{^\textrm{hj}}$} &                $2540$ (1330) & 0.98 (0.49) &    $\cdots$ \\
SN 2004dt           &  1.29 (0.05) &     HV$\phantom{^\textrm{i}}$ &             14.34 (0.10)$\phantom{^\textrm{h}}$ &            HVG$\phantom{^\textrm{hj}}$ &             269.45 $\phantom{00}$(8.34)$\phantom{^\textrm{hj}}$ &                14.70 (0.10)$\phantom{^\textrm{hj}}$ &               $-2850$ (1380) & 1.80 (1.04) &    $\cdots$ \\
SN 2005cf$^\dagger$ &  1.08 (0.03) &      N$\phantom{^\textrm{i}}$ &             10.26 (0.10)$\phantom{^\textrm{h}}$ &            HVG$\phantom{^\textrm{hj}}$ &                         106.69 (149.59)$\phantom{^\textrm{hj}}$ &                10.13 (0.25)$\phantom{^\textrm{hj}}$ &     $910$ $\phantom{0}$(500) & 0.14 (0.09) & 0.53 (0.26) \\
SN 2006X            &  1.10 (0.04) &     HV$\phantom{^\textrm{i}}$ &             15.26 (0.10)$\phantom{^\textrm{h}}$ & HVG$^{\textrm{j}\phantom{\textrm{h}}}$ &  184.80 $\phantom{00}$(5.82)$^{\textrm{j}\phantom{\textrm{h}}}$ &     15.63 (0.06)$^{\textrm{j}\phantom{\textrm{h}}}$ &    $2700$ $\phantom{0}$(410) & 2.04 (1.61) & 1.05 (0.46) \\
SN 2007le           &  1.02 (0.04) &     HV$\phantom{^\textrm{i}}$ &             12.09 (0.10)$\phantom{^\textrm{h}}$ &            HVG$\phantom{^\textrm{hj}}$ &              93.35 $\phantom{0}$(12.65)$\phantom{^\textrm{hj}}$ &                12.77 (0.18)$\phantom{^\textrm{hj}}$ &    $2030$ $\phantom{0}$(140) & 2.36 (0.62) & 0.33 (0.17) \\
SN 2008Q$^\dagger$  &  1.25 (0.08) &     HV$\phantom{^\textrm{i}}$ &             11.09 (0.10)$\phantom{^\textrm{h}}$ & HVG$^{\textrm{j}\phantom{\textrm{h}}}$ &   82.66 $\phantom{0}$(16.22)$^{\textrm{j}\phantom{\textrm{h}}}$ &     11.64 (0.05)$^{\textrm{j}\phantom{\textrm{h}}}$ &   $-2200$ $\phantom{0}$(750) & 0.44 (0.22) &    $\cdots$ \\
SN 2011by           &  1.14 (0.03) &      N$\phantom{^\textrm{i}}$ &             10.35 (0.14)$\phantom{^\textrm{h}}$ &            LVG$\phantom{^\textrm{hj}}$ &              52.83 $\phantom{00}$(8.76)$\phantom{^\textrm{hj}}$ &                10.40 (0.08)$\phantom{^\textrm{hj}}$ &   $-1450$ $\phantom{0}$(170) & 0.66 (0.16) & 0.47 (0.41) \\
\hline \hline
\multicolumn{10}{l}{$^\dagger$Object is part of the low-extinction sample (see text for details).} \\
\multicolumn{10}{l}{$^\textrm{a}$Values taken from Ganeshalingam \etal (in preparation).} \\
\multicolumn{10}{p{6.5in}}{$^\textrm{b}$Classification based on the velocity of the Si~II $\lambda$6355 line near maximum brightness \citep{Wang09}. `HV' = high velocity; `N' = normal. Taken from \citet{Silverman12:BSNIPII}.} \\
\multicolumn{10}{l}{$^\textrm{c}$Velocity of the Si~II $\lambda$6355 feature within 8~d of maximum brightness. Taken from \citet{Silverman12:BSNIPII} unless otherwise noted.} \\
\multicolumn{10}{p{6.5in}}{$^\textrm{d}$Classification based on the velocity gradient of the Si~II $\lambda$6355 line \citep{Benetti05}. `HVG' = high velocity gradient; `LVG' = low velocity gradient; `FAINT' = faint/underluminous. Taken from \citet{Silverman12:BSNIPII} unless otherwise noted.} \\
\multicolumn{10}{p{6.5in}}{$^\textrm{e}$The change in velocity with time, near maximum brightness (i.e., the velocity gradient). Taken from \citet{Silverman12:BSNIPII} unless otherwise noted.} \\
\multicolumn{10}{p{6.5in}}{$^\textrm{f}$The velocity of the Si~II $\lambda$6355 feature extrapolated to $t = 0$~d based on the velocity gradient. Taken from \citet{Silverman12:BSNIPII} unless otherwise noted.} \\
\multicolumn{10}{p{6.5in}}{$^\textrm{g}$Average nebular velocity of the [Fe~II] $\lambda$7155 and [Ni~II] $\lambda$7378 features for all late-time spectra of a given object. The uncertainty is the average difference between the velocity of the two features.} \\
\multicolumn{10}{p{6.5in}}{$^\textrm{h}$Photospheric velocity, Benetti type, velocity gradient, and $v_0$ measured from data presented by \citet{Matheson08}.} \\
\multicolumn{10}{l}{$^\textrm{i}$Classification scheme only applies to spectroscopically normal SNe~Ia.} \\
\multicolumn{10}{p{6.5in}}{$^\textrm{j}$Benetti type, velocity gradient, and $v_0$ measured from BSNIP data as well as data presented by \citet{Blondin12}.} \\
\hline\hline
\end{tabular}
\end{center}
\end{table*}
\normalsize
\setlength{\tabcolsep}{6pt}


==> sn2011by.tex <==
\setlength{\tabcolsep}{0.065in}
\begin{table}
\caption{Journal of spectroscopic observations of SN~2011by.\label{t:sn2011by}}
\begin{center}
\begin{tabular}{lrccc}
\hline\hline
UT Date &Age$^\textrm{a}$&Range (\AA)&Airmass$^\textrm{b}$&Exp (s)\\
\hline
2011 Apr.\ 28.2 & $-11.6$ & 3440--10200	 & 1.05	 & 600 \\
2011 May 4.2 & $-5.6$ & 3440--10200	 & 1.06	 & 600 \\
2011 May 6.2 & $-3.7$ & 3440--10200	 & 1.05	 & 600 \\
2011 May 10.2 & 0.3 & 3438--10196	 & 1.06	 & 600 \\
2011 May 14.2 & 4.3 & 3456--10200	 & 1.07	 & 600 \\
2011 May 22.3 & 12.3 & 3464--10200	 & 1.15	 & 600 \\
2011 May 25.3 & 15.4 & 3436--10200	 & 1.27	 & 600 \\
% 2011 Jun.\ 08.3	 & 3436--10200	 & 1.33	 & 600 \\
% 2011 Jun.\ 30.2	 & 3448--10200	 & 1.29	 & 1000 \\
\hline
2011 Dec.\ 2.6$^\textrm{c}$ & 206 & 3400--10138	 & 1.50	 & 450 \\
2012 Mar.\ 15.5$^\textrm{c}$ & 310  & 3400--10200	 & 1.32	 & 900 \\
\hline\hline
\multicolumn{5}{p{3.1in}}{$^\textrm{a}$Rest-frame days relative to the date of $B$-band maximum brightness, 2011~May~9.9 (see Section~\ref{ss:sn2011by}).} \\
\multicolumn{5}{p{3.1in}}{$^\textrm{b}$Airmass at midpoint of exposure.} \\
\multicolumn{5}{p{3.1in}}{$^\textrm{c}$These observations used LRIS \citep{Oke95} on the 10-m Keck~I telescope. The others used the Kast spectrograph on the Lick 3-m Shane telescope \citep{Miller93}.} \\
\end{tabular}
\end{center}
\end{table}
\setlength{\tabcolsep}{6pt}


==> v_neb.tex <==
\setlength{\tabcolsep}{0.07in}
\onecolumn
\begin{landscape}
\begin{center}
\begin{longtable}{lcrrrr|lcrrrr}
\caption{\hbox to 4.1in{Nebular feature measurements. All FWHMs and velocities are in \kms.}}\label{t:v_neb} \\[-2ex]
\hline \hline
   &    & \multicolumn{1}{c}{FWHM} & \multicolumn{1}{c}{Velocity} & \multicolumn{1}{c}{Velocity} & Velocity\hspace{.13in} & & & \multicolumn{1}{c}{FWHM} & \multicolumn{1}{c}{Velocity} & \multicolumn{1}{c}{Velocity} & \multicolumn{1}{c}{Velocity} \\
SN Name & Phase$^\textrm{a}$ & \multicolumn{1}{c}{[Fe III] $\lambda$4701} & \multicolumn{1}{c}{[Fe III] $\lambda$4701} & \multicolumn{1}{c}{[Fe II] $\lambda$7155} & [Ni II] $\lambda$7378 & SN Name & \multicolumn{1}{c}{Phase$^\textrm{a}$} & \multicolumn{1}{c}{[Fe III] $\lambda$4701} & \multicolumn{1}{c}{[Fe III] $\lambda$4701} & \multicolumn{1}{c}{[Fe II] $\lambda$7155} & \multicolumn{1}{c}{[Ni II] $\lambda$7378} \\
\hline
\endfirsthead
\multicolumn{12}{c}{{\tablename} \thetable{} --- Continued} \\
\hline \hline
   &    & \multicolumn{1}{c}{FWHM} & \multicolumn{1}{c}{Velocity} & \multicolumn{1}{c}{Velocity} & Velocity\hspace{.13in} & & & \multicolumn{1}{c}{FWHM} & \multicolumn{1}{c}{Velocity} & \multicolumn{1}{c}{Velocity} & \multicolumn{1}{c}{Velocity} \\
SN Name & Phase$^\textrm{a}$ & \multicolumn{1}{c}{[Fe III] $\lambda$4701} & \multicolumn{1}{c}{[Fe III] $\lambda$4701} & \multicolumn{1}{c}{[Fe II] $\lambda$7155} & [Ni II] $\lambda$7378 & SN Name & \multicolumn{1}{c}{Phase$^\textrm{a}$} & \multicolumn{1}{c}{[Fe III] $\lambda$4701} & \multicolumn{1}{c}{[Fe III] $\lambda$4701} & \multicolumn{1}{c}{[Fe II] $\lambda$7155} & \multicolumn{1}{c}{[Ni II] $\lambda$7378} \\
\hline
\endhead

\hline \hline
\multicolumn{12}{l}{Continued on Next Page\ldots} \\
\endfoot

\hline \hline
\endlastfoot

SN 1989M               & 146.8 &    15000 &  $-2800$ &    $660$ &    $450$ &
SN 1991T               & 112.2 &    14300 &  $-2710$ & $\cdots$ & $\cdots$ \\
SN 1991T               & 318.4 &    17200 &    $810$ & $\cdots$ & $\cdots$ &
SN 1991T               & 347.2 &    17000 &   $1810$ & $\cdots$ & $\cdots$ \\
SN 1991bg              & 161.9 &     3200 &  $-1840$ & $\cdots$ & $\cdots$ &
SN 1992G               & 110.8 &    14700 &  $-3000$ & $\cdots$ & $\cdots$ \\
SN 1992G               & 111.9 &    14700 &  $-3130$ & $\cdots$ & $\cdots$ &
SN 1992G               & 126.8 &    16000 &  $-2990$ & $\cdots$ & $\cdots$ \\
SN 1993Z               & 112.5 &    15100 &  $-2120$ & $\cdots$ & $\cdots$ &
SN 1993Z               & 132.4 &    15000 &  $-2120$ & $\cdots$ & $\cdots$ \\
SN 1993Z               & 144.3 &    14800 &  $-1230$ & $\cdots$ & $\cdots$ &
SN 1993Z               & 161.2 &    14400 &  $-1350$ &   $1820$ &   $1180$ \\
SN 1993Z               & 200.8 &    15300 &  $-2880$ &   $1900$ &   $3660$ &
SN 1993Z               & 232.7 &    14400 &   $-720$ &   $1000$ &   $2390$ \\
SN 1994D               & 114.7 &    15400 &  $-3010$ &  $-2280$ &  $-1150$ &
SN 1994ae              & 144.0 &    14500 &  $-2430$ & $\cdots$ & $\cdots$ \\
SN 1994ae              & 218.6 &    12200 &   $-890$ & $\cdots$ & $\cdots$ &
SN 1998bp              & 139.4 &     8700 &  $-3490$ & $\cdots$ & $\cdots$ \\
SN 1998bp              & 163.1 &    10600 &  $-2340$ & $\cdots$ & $\cdots$ &
SN 1998bu              & 235.1 &    15600 &  $-1030$ &  $-1890$ &   $-790$ \\
SN 1998bu              & 279.0 &    16400 &  $-2040$ &  $-1710$ &  $-1430$ &
SN 1998bu              & 338.7 &    22200 &   $-650$ &  $-2640$ &  $-2330$ \\
SN 1998es              & 106.0 &    13500 &  $-3790$ & $\cdots$ & $\cdots$ &
SN 1999aa              & 255.9 &    16700 &  $-1030$ &    $830$ &    $690$ \\
SN 1999aa              & 281.5 &    18500 &    $520$ & $\cdots$ & $\cdots$ &
SN 1999ac              & 116.9 &    10300 &  $-2200$ & $\cdots$ & $\cdots$ \\
SN 1999by              & 183.5 &     9500 &  $-1440$ & $\cdots$ & $\cdots$ &
SN 1999cw              & 104.6 &    14400 &  $-2920$ & $\cdots$ & $\cdots$ \\
SN 1999cw              & 132.1 &    13600 &  $-2410$ & $\cdots$ & $\cdots$ &
SN 1999gh              & 118.0 &    12200 &  $-4200$ &   $1290$ &   $1840$ \\
SN 2001ep              & 114.9 &    12400 &  $-3370$ & $\cdots$ & $\cdots$ &
SN 2002bo              & 227.4 &    16600 &  $-1620$ &   $2330$ &   $2530$ \\
SN 2002cs              & 119.0 &    15500 &  $-3810$ & $\cdots$ & $\cdots$ &
SN 2002cs              & 143.5 &    15000 &  $-4280$ & $\cdots$ & $\cdots$ \\
SN 2002cs              & 172.2 &    15800 &  $-3720$ & $\cdots$ & $\cdots$ &
SN 2002dp              & 103.1 &    14300 &  $-4080$ & $\cdots$ & $\cdots$ \\
SN 2002dp              & 134.7 &    13800 &  $-2630$ & $\cdots$ & $\cdots$ &
SN 2002fk              & 148.7 &    14600 &  $-2650$ &  $-1370$ &  $-2750$ \\
SN 2003gs              & 199.5 &    14700 &  $-2630$ &   $3870$ &   $1210$ &
SN 2004bv              & 135.2 &    14200 &  $-3300$ & $\cdots$ & $\cdots$ \\
SN 2004bv              & 161.7 &    14300 &  $-2530$ & $\cdots$ & $\cdots$ &
SN 2004dt              & 109.2 &    13600 &  $-4970$ & $\cdots$ & $\cdots$ \\
SN 2004dt              & 168.9 & $\cdots$ & $\cdots$ &  $-1470$ &  $-4220$ &
SN 2005cf              & 317.1 &    15400 &   $-530$ &    $410$ &   $1400$ \\
SN 2005ke              & 362.1 &    10500 &   $-430$ & $\cdots$ & $\cdots$ &
SN 2006D               & 126.5 &    14200 &  $-3320$ & $\cdots$ & $\cdots$ \\
SN 2006X               & 126.3 &    15200 &  $-2970$ &   $3420$ &   $2320$ &
SN 2006X               & 275.9 &    19300 &   $1210$ &   $2610$ &   $2730$ \\
SN 2006X               & 358.4 &    23700 &  $-3290$ &   $1960$ &   $3180$ &
SN 2007af              & 113.8 &    13300 &  $-2920$ & $\cdots$ & $\cdots$ \\
SN 2007af              & 121.7 &    13300 &  $-2790$ & $\cdots$ & $\cdots$ &
SN 2007af              & 144.6 &    13100 &  $-3170$ & $\cdots$ & $\cdots$ \\
SN 2007af              & 158.5 &    13600 &  $-3550$ & $\cdots$ & $\cdots$ &
SN 2007fb              & 100.9 &    13700 &  $-3590$ & $\cdots$ & $\cdots$ \\
SN 2007gi              & 153.3 &    15800 &  $-1440$ & $\cdots$ & $\cdots$ &
SN 2007le              & 304.7 &    16700 &   $-230$ &   $2160$ &   $1890$ \\
SN 2007sr              & 135.7 &    13700 &  $-2280$ & $\cdots$ & $\cdots$ &
SN 2008Q               & 199.3 &    15700 &  $-1860$ &  $-2940$ &  $-1450$ \\
SN 2011by              & 206.1 &    14500 &  $-2260$ &  $-1350$ &  $-1470$ &
SN 2011by              & 309.7 &    15300 &   $-280$ &  $-1210$ &  $-1750$ \\
\hline \hline
\multicolumn{12}{p{9.2in}}{$^\textrm{a}$Phases of spectra are in rest-frame days relative to $B$-band maximum brightness using the heliocentric redshift and photometry reference presented in Table~1 of \citet{Silverman12:BSNIPI} and Section~\ref{ss:sn2011by} for SN~2011by.} \\
\end{longtable}
\end{center}
\end{landscape}
\twocolumn
\setlength{\tabcolsep}{6pt}

